Features and New Physical Scales in Primordial Observables: Theory and Observation

All cosmological observations to date are consistent with adiabatic, Gaussian and nearly scale invariant initial conditions. These findings provide strong evidence for a particular symmetry breaking pattern in the very early universe (with a close to vanishing order parameter, $\epsilon$), widely accepted as conforming to the predictions of the simplest realizations of the inflationary paradigm. However, given that our observations are only privy to perturbations, in inferring something about the background that gave rise to them, it should be clear that many different underlying constructions project onto the same set of cosmological observables. Features in the primordial correlation functions, if present, would offer a unique and discriminating window onto the parent theory in which the mechanism that generated the initial conditions is embedded. In certain contexts, simple linear response theory allows us to infer new characteristic scales from the presence of features that can break the aforementioned degeneracies among different background models, and in some cases can even offer a limited spectroscopy of the heavier degrees of freedom that couple to the inflaton. In this review, we offer a pedagogical survey of the diverse, theoretically well grounded mechanisms which can imprint features into primordial correlation functions in addition to reviewing the techniques one can employ to probe observations. These observations include cosmic microwave background anisotropies and spectral distortions as well as the matter two and three point functions as inferred from large-scale structure and potentially, 21 cm surveys.

==> LSS.tex <==
As long as the amplitude of matter density fluctuations, $\delta_\mathrm{m}/\bar{\delta}_\mathrm{m} \ll 1$, matter fluctuations of different wavenumbers evolve independently and the power spectrum of the matter distribution is related to the primordial power spectrum of curvature fluctuations by
\begin{equation}
\mathcal{P}_\mathrm{m} (k,z) = \int \mathrm{d}k' \; T_\mathrm{m}(k,k',z) \mathcal{P_R}(k) \approx T^\mathrm{lin}_\mathrm{m} (k,z) \mathcal{P_R}(k),
\end{equation}
where $T^\mathrm{(lin)}_\mathrm{m}$  is the (linear) matter transfer function.  Compared to the CMB, where information about the fluctuations is fundamentally limited to the two-dimensional surface of last scattering, the distribution of matter can be probed in three dimensions.  This has two important consequences:  firstly, one gains sensitivity to the time evolution of the power spectrum which is very helpful in disentangling primordial features from non-primordial ones.\footnote{Consider, e.g., the suppression of power on small scales due to the free-streaming effect of massive neutrinos.  This is a time-dependent effect that becomes more pronounced at later times, as opposed to a primordial power spectrum suppression, which will show up equally at all redshifts.}  Secondly, the ability to detect density fluctuations along the line of sight results in an increase of the number of observable modes for a given wavenumber, greatly reducing the uncertainty due to cosmic variance.

Despite the ability to recover some 3-dimensional information, a finite-volume survey will still be subject to a limited resolution in $k$.  Observations allow us to construct an estimate of the power spectrum in band powers $\mathcal{P}_i$~\cite{Feldman:1993ky}, which are related to the true power spectrum in terms of a convolution with a set of window functions $\mathcal{W}_i(k)$:
\begin{equation}
\mathcal{P}_i(k_i) = \int \mathrm{d}k' \; \mathcal{W}_i(k-k') \mathcal{P}(k').
\end{equation}
Depending on the survey geometry, one can construct an optimal set of window functions that are as narrow and uncorrelated as possible without compromising the variance in $\mathcal{P}$~\cite{Tegmark:1995xxx}.  For a volume-limited all-sky survey out to a distance $R$, the optimal window function in the large-scale limit is given by 
\begin{equation}
\mathcal{W}(k) = 4 \pi R \left( \frac{\sin k R}{\pi^2 - k^2 R^2} \right)^2,
\end{equation}
whose width scales like $R^{-1}$.


\subsection{Galaxy surveys}


Alternatively, angular power spectrum plus tomography (redshift binning), subject to same smearing as CMB, but redshift bins -> independent fluctuations -> beat down cosmic variance

Main issues: galaxy bias, redshift space distortions, non-linear evolution mixes modes, wiping out features

Presently not able to compete with CMB.  However, unlike CMB, 3-d information can be obtained. 
Possible to improve on CMB with next generation observations:  large volume galaxy surveys (10 years from now), 21~cm surveys (20? years from now).

Using galaxies as tracers, one can realistically expect to map out the matter distribution up to a redshift of $~2$.  


\subsection{21 cm surveys}
A more radical idea is to use neutral hydrogen as a tracer of the matter distribution and reconstruct its three-dimensional structure by measuring emission or absorption due to the 21~cm hydrogen spin flip~\cite{Scott:1990bla}.  Using the emission signal caused by reionisation~\cite{McQuinn:2005hk}, a redshift range of $6 \lesssim z \lesssim 20$ may be accessible.

Foregrounds are a big issue.

To date, no cosmological signal has been detected, but experimental programmes are on the way to evaluate the potential of this observable.

Tianlai project~\cite{Chen:2012xu}, designed to measure the BAO scale at different redshifts.  In the more distant future, an experiment such as the Fast Fourier Transform Telescope~\cite{Tegmark:2008au}.


\subsection{Higher order correlators \label{sec:hoc}}
Higher order statistics, presumably?

==> section_four.tex.v1 <==
In the previous section, we saw that there are a wide range of theoretical scenarios that can lead to features in the primordial power spectrum, which begs the question: are any of these realised in nature?  Addressing this requires us to confront the theoretical predictions with experimental evidence. However, our quest for features is not completely straightforward -- nature has endeavoured to muddle the waters in several nefarious ways.

First of all, the quantities predicted by theory, i.e. the statistical properties of the primordial curvature perturbation are not directly observable;  we can neither access anything primordial, nor can we ``see'' curvature perturbations.
At best, we can gain indirect information by measuring derived quantities, such as matter density perturbations or anisotropies in the cosmic microwave background that have evolved from the initial state.  In general, the relation of the primordial spectrum to actual observables depends on additional cosmological parameters unrelated to inflation (e.g. the baryon and dark matter densities, the Hubble parameter, the optical depth at recombination etc.) whose effect may, in some cases, be confused with a feature.

Secondly, the generation of initial perturbations is a stochastic process, and quantities like the primordial curvature perturbation or the matter density fluctuation are random fields. Exact, deterministic theoretical predictions of, for example, the power spectrum of these fields can only be made for ensemble averages (or equivalently, their average over an infinite volume).   When it comes to observing the universe however, we are limited to finite volumes. In this case, the theoretical power spectrum of the field over this volume becomes a random variable: its expectation value is given by the ensemble average, but it is subject to a sampling variance (in this context also known as {\it cosmic variance}) which depends on the size and shape of the volume observed. Note that sampling variance is an intrinsic theoretical uncertainty; the only way to reduce it is by increasing the observed volume.  This means that even if we had a perfect measurement, the power spectrum constructed from these data will be subject to a scatter which can obscure or even mimic the presence of features.

Thirdly, the scatter is compounded by statistical uncertainties that all realistic measurements are subject to (e.g., due to finite detector resolution, detector noise, shot noise, etc.). This problem can at least in principle be overcome with better technological means; once these uncertainties are reduced to below the level of the sampling variance, they cease to be relevant.

Finally, there is only the finite window of wavenumbers accessible to observation. The size of the universe's particle horizon today sets a lower limit on the wavenumber of observable perturbations $k \gtrsim 2 \times 10^{-4}$~Mpc$^{-1}$. The upper limit depends on the probe: structures at low redshifts ($z \lesssim 1$) have undergone non-linear evolution on scales $k \gtrsim \mathcal{O}(10^{-1})$~Mpc$^{-1}$, where mode-coupling has erased all but the broadest features.  At higher redshifts non-linear evolution becomes less of an issue, though in the case of the CMB, the original signal is significantly suppressed by Silk-damping from photon diffusion \cite{Silk1968} and tends to be swamped by foregrounds beyond $k \gtrsim \mathcal{O}(10^{-1})$~Mpc$^{-1}$. For other probes of the (matter) power spectrum such as 21~cm tomography, it may in principle be possible to see linearly coupled modes out to $k \approx \mathcal{O}(10^{2})$~Mpc$^{-1}$ \cite{Loeb:2003ya, Furlanetto:2006jb, vanHaarlem:2013dsa, Rawlings:2004wk}. Therefore, given presently available data and being generous, the observable window spans a good four orders of magnitude in $k$, corresponding to roughly 10 $e$-foldings of inflation; features produced outside this range are hidden from our direct view. However, as previously mentioned and as we shall elaborate upon further below, it will soon be possible to open the window on the shorter wavelength modes by tapping the information contained in spectral distortions and 21~cm surveys, the former potentially allowing us a window onto comoving scales up to  $k \approx \mathcal{O}(10^{4})$~Mpc$^{-1}$ \cite{PRISM2013WPII, Chluba2012inflaton}. This would add another 5 $e$-foldings of inflation to the picture.

So what options do we have to get a handle on the primordial power spectrum?  In this section, we will cover the most direct approach:  measuring inhomogeneities (or anisotropies) of the universe's constituents and relating them to primordial perturbations. All energy components of the  $\Lambda$CDM model except for dark energy (i.e., photons, neutrinos, baryons and cold dark matter), have inhomogeneities, making them potentially useful sources of information about the initial fluctuations. Out of these, we can exclude the perturbations of the neutrino background: while in principle a good probe of the primordial power spectrum~\cite{Hannestad:2009xu}, cosmic background neutrinos are elusive creatures and although their direct detection may be within reach with current technology \cite{Ringwald:2009bg, Betts:2013uya, Kaboth:2010kf}, a detection of their anisotropies is unlikely in the foreseeable future. This leaves us with photon and matter perturbations. The latter can be revealed either via visible tracers such as galaxies and neutral hydrogen gas, or through their weak gravitational lensing effect on background sources.  The perturbations of the photons (or, more precisely, of the baryon-photon fluid around decoupling) can be directly observed in the form of temperature and polarisation anisotropies of the cosmic microwave background. Furthermore, looking beyond anisotropies, one may potentially be able to constrain or even detect primordial features with just the monopole through distortions to the CMB spectrum. We elaborate upon this intriguing idea in detail in Section~\ref{sec:spectraldistortions}.

\subsection{Cosmic microwave background anisotropies}

Currently, the by far most sensitive probe for features, and the only one able to reach the lower limit of the observable wavenumber window, are the anisotropy measurements of the cosmic microwave background radiation. From the observed maps of the CMB's temperature fluctuations and polarisation, one can extract the \textit{angular power spectra} $\widehat{C}_\ell^{XY}$, where $X,Y \in \left\{\mathrm{T,E} \right\}$.\footnote{The $B$-component of the CMB polarisation is not sourced by scalar perturbations at linear order and hence not helpful in probing $\mathcal{P_R}(k)$.} These are defined as follows-- first consider expanding the observed temperature anisotropies in the sky in terms of spherical harmonics
\eq{dtot}{\frac{\Delta \widehat T}{\widehat T}(\vec n) = \sum_{\ell m} a^T_{\ell m} Y_{\ell m}(\vec n) }
where $\vec n$ is a unit vector on the sphere and where the $a^T_{\ell m}$ are stochastic variables. Were we to presume statistical isotropy, it can be shown that the average over an ensemble of universes satisfies
\eq{angdef}{\langle a^X_{\ell m} a^{Y*}_{\ell' m'} \rangle = C^{XY}_\ell \delta_{\ell\ell'}\delta_{m m'}}
which defines the $C^{XY}_\ell$'s as the angular auto/cross correlation function for the variables X/Y in question. The observed $\widehat{C}_\ell^{XY}$ are to be compared to the theoretical prediction, $C_\ell^{XY} $.  In the absence of initial vector and tensor perturbations, to linear order, the $C_\ell^{XY} $ are determined by the scalar contributions to the temperature and E-polarisation auto- and cross-correlation angular power spectra, which can be expressed in terms of the power spectrum of the comoving curvature mode as \cite{Lesgourgues:2013qba}
\eq{eq:cls}{\boxed{C_\ell^{XY} = \frac{1}{2\pi^2} \int \mathrm{d}\ln k \; \Delta^X_\ell(k,\tau_0) \Delta^Y_\ell(k,\tau_0) \mathcal{P_R}(k).}}
The transfer functions $\Delta^X_\ell$ are integrals over comoving time $\tau$,
\eq{eq:transfer}{\Delta^X_\ell(k,\tau_0) = \int_{\tau_{\mathrm{ini}}}^{\tau_0} \mathrm{d}\tau \; S^X(k,\tau) j_\ell(k(\tau-\tau_0)),}
with a geometrical part given by $j_\ell$, the spherical Bessel functions of order $\ell$, and the source functions $S^X$ which contain the dependence on non-primordial cosmological parameters such as the matter and baryon densities. The source functions are typically evaluated using a Boltzmann code (see \cite{Durrer:1127831} for a detailed derivation and \cite{Mukhanov:2003xr} for a reasonably accurate analytic understanding up to $\ell \sim 200$). The $C_\ell^{XY}$ thus computed are ensemble averages; for observations of the full sky, 
we can estimate the angular cross/auto power spectra by constructing the following \textit{estimator}:
\eq{}{\widehat C^{XY}_\ell = \frac{1}{2\ell + 1}\sum_m a_{\ell m}^X a_{\ell m}^{Y*}.}
From (\ref{angdef}) we see that although this estimator is \textit{unbiased} in the sense that
\eq{}{\langle \widehat C_\ell^{XY}\rangle = C_\ell^{XY},}
it has a non-zero (cosmic) variance~\cite{Martinez:1339567},
\begin{eqnarray}\label{cosvar}
{\rm var} ~\widehat C^{XY}_\ell &:=& \langle \widehat C_\ell^{XY} \widehat C_\ell^{XY} \rangle - \langle \widehat C_\ell^{XY} \rangle\langle\widehat C_\ell^{XY} \rangle\\
\nonumber &=& \frac{1}{(2\ell +1)^2} \sum_{m m'} \langle a^X_{\ell m}a^{Y*}_{\ell m} a^X_{\ell m'}a^{Y*}_{\ell m'} \rangle - {C_\ell^{XY}}^2\\ &=& \nonumber \frac{1}{(2\ell +1)^2} \sum_{m m'} \left[\langle a^X_{\ell m}a^{X}_{\ell m'}\rangle\langle a^{Y*}_{\ell m}a^{Y*}_{\ell m'} \rangle + \langle a^X_{\ell m}a^{Y*}_{\ell m'}\rangle\langle a^{X}_{\ell m'}a^{Y*}_{\ell m} \rangle \right]\\ &=& \nonumber \frac{1}{2\ell + 1}\left[C_\ell^{XX}C_\ell^{YY} + {C_\ell^{XY}}^2\right],
\end{eqnarray}
where the third line follows from the second by presuming that the $a_{\ell m}$'s satisfy almost Gaussian statistics and that they correspond to real variables (so that $a^{X*}_{\ell m} = a^X_{\ell -m}$). Therefore for the auto-correlation functions we have
\eq{}{\boxed{ {\rm var} ~\widehat C_\ell^{XX} = \frac{2}{2\ell + 1} {C_\ell^{XX}}^2}}
That is to say, the $\widehat{C}_\ell^{XY}$ are random variables with mean $C_\ell^{XY}$ and subject to a cosmic (sampling) variance given by (\ref{cosvar}). Realistic experiments will not be able to observe the CMB over the full sky, either due to experimental design (e.g., for ground-based or balloon experiments) or the need to mask areas where foregrounds cannot be removed, such as the galactic plane.
If only a fraction $f_\mathrm{sky}$ of the sky is covered, the cosmic variance will scale roughly with a factor $1/f_\mathrm{sky}$, and the inferred $\widehat{C}_\ell^{XY}$ are no longer uncorrelated.

Looking at equation~(\ref{eq:cls}), schematically, the angular power spectrum is a convolution of the primordial power spectrum with a window function, given by the product of two transfer functions. Invariably, this convolution leads to a loss of information: features in $\mathcal{P_R}(k)$ will be smeared out to a certain degree and show up less prominently in ${C}_\ell$.\footnote{Besides the smearing due to the geometrical projection, the observed angular power spectra are themselves subject to further convolutions due to (i) the effects of weak gravitational lensing on the CMB~\cite{Lewis:2006fu}, and (ii) the aberration caused by the proper motion of the observer with respect to the CMB rest frame~\cite{Jeong:2013sxy}.}   If the characteristic width of a feature in $k$-space exceeds the width of the window function on the corresponding scales, its amplitude in the angular power spectrum will be approximately suppressed by the inverse ratio between the two.   Thus, provided a sufficiently high frequency, even a relative modulation of the primordial spectrum of $\mathcal{O}(1)$ could be hidden in the angular power spectrum-- though the deviation from linear evolution required to produce such a large modulation is likely going to induce a strong signal in higher order correlations (see Section~\ref{sec:hoc}).  


\subsubsection{CMB temperature anisotropies}

\begin{figure}[t]
\center
\includegraphics[height=.90\textwidth,angle=270]{figures/temp_delta.pdf}
\caption{Temperature auto-correlation angular power spectrum window functions for multipoles \mbox{$\ell = 2,20,200$}~and~$2000$, normalised to their respective maxima.\label{fig:temp_delta}}
\end{figure}

We show the window functions of the temperature anisotropies for multipoles \mbox{$\ell = 2, 20, 200$}  and $2000$ in Figure~\ref{fig:temp_delta}.  Their rapid oscillations are due to the Bessel functions, and changing the later-time cosmology will modify the envelopes.  
As one goes to higher multipoles, the log-width of the window functions decreases from about 0.4 at $\ell = 2$ to 0.045 at $\ell = 2000$ (assuming the Planck best-fit $\Lambda$CDM late-time cosmology). At multipoles $\ell \gtrsim 2000$, the primary CMB temperature signal becomes rapidly subdominant to secondary microwave anisotropies, e.g., from point sources, the cosmic infrared background or the Sunyaev-Zeldovich effects \cite{Zeldovich1969, Sunyaev1980}, which are which are much less sensitive to the presence of features.  Thus the range of wavenumbers over which the CMB temperature spectrum is sensitive to features is given roughly by the interval $0.0002~\mathrm{Mpc}^{-1} \lesssim k \lesssim 0.15~\mathrm{Mpc}^{-1}$. This range has in fact been almost entirely covered at the cosmic variance limit by the Planck mission~\cite{Adam:2015rua} (see Figure~\ref{fig:plonk_cls}).

\begin{figure}[t]
\center
\includegraphics[height=.90\textwidth,angle=270]{figures/PlanckTT.pdf}
\caption{\textit{Top:} Planck full mission measurement of the angular power spectrum of the temperature autocorrelation of the CMB~\cite{Adam:2015rua}. \textit{Bottom:} Residuals in units of standard deviations with respect to the best-fit $\Lambda$CDM model. For $\ell > 30$, the power spectrum is binned.  The error bars denote the variance due to sampling error and experimental uncertainties due to, e.g., detector noise, component separation or beam errors. \label{fig:plonk_cls}}
\end{figure}

\subsubsection{CMB polarisation anisotropies}

\begin{figure}[t]
\center
\includegraphics[height=.90\textwidth,angle=270]{figures/epol_delta.pdf}
\caption{Same as Fig.~\ref{fig:temp_delta}, for the $E$-polarisation autocorrelation.\label{fig:epol_delta}}
\end{figure}

The temperature anisotropies of the cosmic microwave background are not the only source of information one can obtain from the decoupling era.  The CMB is weakly linearly polarised due to Thomson scattering (the low energy limit of Compton scattering) of the CMB photons during decoupling~\cite{Bond:1984fp, Hu:1997hv}, sourced by the local quadrupole anisotropy in the incident radiation intensity field.  Measuring the angular power spectrum of the $E$-component of the CMB polarisation is a powerful complementary tool in the search for features in the primordial spectrum and potentially even surpasses the temperature in terms of sensitivity.  Not only is the small-scale polarisation signal to a lesser degree subject to foreground contamination, with the primary signal dominant up to $\ell \sim 4000$~\cite{Seiffert:2006vh,Bock:2008ww}, the polarisation window functions for a given multipole are also narrower than the corresponding temperature window functions (see Figure~\ref{fig:epol_delta})~\cite{Hu:2003vp}, leading to more sharply defined features in the observable $E$-autocorrelation spectrum. Here, the log-width of the window functions ranges from roughly 0.13 at $\ell = 2$ to 0.03 at $\ell = 2000$.
It should be noted however, that on the largest scales ($\ell \lesssim 20$), the polarisation power spectrum is dominated by the contribution generated during reionisation.  At those scales, features in the $EE$-spectrum could also imply a deviation from the commonly assumed nearly instantaneous reionisation model, rather than point to a primordial origin.

Mortonson et al.~\cite{Mortonson:2009qv}, for example, considered a putative oscillatory feature around $k = 2-5 \times 10^{-3}~\mathrm{Mpc}^{-1}$ (corresponding to $20 \lesssim \ell \lesssim 40$) which improves the fit to CMB temperature data by $2 \Delta \ln \mathcal{L}^{TT} \approx 10$ (see Sect. \ref{sec:statistics}) for a definition of the former quantity).  In a cosmic-variance limited measurement of the $E$-polarisation autocorrelation spectrum, such a feature can be expected to lead to $2 \Delta \ln \mathcal{L}^{EE} \approx 60$ when the reionisation history is known, and $\sim 30$ if it is allowed to freely vary. Since the $EE$-spectrum is suppressed by a few orders of magnitude with respect to the temperature spectrum, measuring it demands much higher instrumental sensitivity. Unlike Planck's temperature data, its polarisation data is not limited by cosmic variance (but nonetheless adds useful information at intermediate scales~\cite{Mortonson:2009qv,Ade:2015lrj}).  An all-sky cosmic variance-limited measurement to much smaller scales is feasible with current technology and several experimental designs have been proposed~\cite{Bock:2008ww,Bouchet:2011ck,Andre:2013afa}. Although none of the former have been selected for funding to date, ground based and sub-orbital CMB polarisation measurements (which either by themselves \cite{Lazear:2014bga} or taken in combination \cite{Ahmed:2014ixy, Niemack:2010wz, 2014arXiv1407.2973B, 2012SPIE.8452E..1EA, Kermish:2012eh, Keating:2011iq, Filippini:2011ds, Fraisse:2011xz, Eimer:2012ny, ReichbornKjennerud:2010ja, MacDermid:2014wca, Matsumura:2013aja,Kogut:2011xw, Ogburn:2012ma}, promise almost full sky coverage) remain one of the most promising future avenues for the detection of features, especially on the largest scales.

\subsection{The matter power spectrum}
Long after recombination, the initial inhomogeneities imprinted in the CMB evolved into the scaffolding upon which large scale structures formed. The central quantity to describe the statistical properties of these inhomogeneities (which are matter density fluctuations around the mean density) given by $\delta \rho_\mathrm{m}/\bar{\rho}_\mathrm{m} \equiv \delta_\mathrm{m}$, is the matter power spectrum $\mathcal{P}_\mathrm{m} (k,z)$, defined via
\begin{equation}
\langle \delta_\mathrm{m}(\mathbf{k},z) \delta_\mathrm{m}(\mathbf{k}',z) \rangle \equiv \frac{2\pi^2}{k^3}  \delta^3(\mathbf{k}-\mathbf{k}') \; \mathcal{P}_\mathrm{m}(k,z).
\end{equation}
As long as the fluctuation amplitude is small, $\delta_\mathrm{m} \ll 1$, matter fluctuations of different wavenumbers evolve independently and $\mathcal{P}_\mathrm{m}$ is directly related to the primordial power spectrum of curvature fluctuations via
\begin{equation}
\mathcal{P}_\mathrm{m} (k,z) = \int \mathrm{d}k' \; T_\mathrm{m}(k,k',z) \mathcal{P_R}(k) \approx T^\mathrm{lin}_\mathrm{m} (k,z) \mathcal{P_R}(k),
\end{equation}
where $T^\mathrm{(lin)}_\mathrm{m}$  is the (linear) matter transfer function containing the dependence on the intervening cosmology.  Compared to the CMB where information about the fluctuations is fundamentally limited to the two-dimensional surface of last scattering, the distribution of matter can be probed in three dimensions.  This has two important consequences: firstly, one gains sensitivity to the time evolution of the power spectrum which is very helpful in disentangling primordial features from non-primordial ones\footnote{Consider, e.g., the suppression of power on small scales due to the free-streaming effect of massive neutrinos.  This is a time-dependent effect that becomes more pronounced at later times, as opposed to a primordial power spectrum suppression, which will show up equally at all redshifts.}.  Secondly, the ability to detect density fluctuations along the line of sight results in an increase of the number of observable modes for a given wavenumber, greatly reducing the uncertainty due to sample variance, with $\mathrm{var}\, \mathcal{P}_\mathrm{m}(k) \propto V^{-1} k^{-2} \mathcal{P}_\mathrm{m}(k)$ for a given volume~$V$.

Despite the ability to recover some 3-dimensional information, a finite-volume survey will still be subject to a limited resolution in $k$.  This becomes apparent when one considers the spatial correlation function, which is related to the power spectrum by a Fourier transform. Take for instance a sinusoidal modulation of $\mathcal{P_R}(k)$ with frequency $\omega$: in the correlation function this corresponds to a spike at a length scale $l \propto \omega$.  If for a given frequency $\omega$ the survey volume is too small to accommodate this length scale, it will not be possible to see the spatial correlation and thus one also will not be able to resolve the modulation.
As a consequence, observations of the matter perturbations over a finite volume only allow us to construct an estimate of the power spectrum in band powers $\mathcal{P}_i$~\cite{Feldman:1993ky}, which are related to the full power spectrum in terms of a convolution with a set of window functions $\mathcal{W}_i(k)$:
\begin{equation}
\boxed{\mathcal{P}_i(k_i) = \int \mathrm{d}k' \; \mathcal{W}_i(k-k') \mathcal{P}(k').}
\end{equation}
Depending on the survey geometry, one can construct an optimal set of window functions that are as narrow and uncorrelated as possible without compromising the variance in $\mathcal{P}$~\cite{Tegmark:1995xxx}.  For a volume-limited all-sky survey out to a distance $R$, the optimal window function in the large-scale limit is given by 
\begin{equation}
\label{eq:window}
\mathcal{W}(k) = 4 \pi R \left( \frac{\sin k R}{\pi^2 - k^2 R^2} \right)^2,
\end{equation}
whose width scales like $R^{-1}$.  This effect is illustrated in the bottom panel of Fig.~\ref{fig:wiggle_delta}, for effective survey volumes $R^3 = 1 \; \mathrm{Gpc}^3 h^{-3}$, representative of current surveys (e.g., SDSS LRG~\cite{Reid:2009xm}), and $R^3 = 50 \; \mathrm{Gpc}^3 h^{-3}$, which is within reach of upcoming projects like the Large Synoptic Survey Telescope (LSST)~\cite{Abell:2009aa} or Euclid~\cite{Laureijs:2011gra}.  In the example here, the feature at large scales cannot be resolved.  The width of $\mathcal{W}$ for a $R \sim \mathcal{O}(1)$~Gpc is $\mathcal{O}(0.001) \; h\, \mathrm{Mpc}^{-1}$, so structures in the spectrum with a smaller characteristic size $\Delta k$ will be erased.

\begin{figure}[t]
\center
\includegraphics[height=.90\textwidth,angle=270]{figures/pkcl.pdf}
\caption{Relative fluctuations for two example primordial features ({\it top}) and the corresponding modulation of the CMB temperature and $E$-polarisation angular power spectra ({\it centre}, thin black lines mark the cosmic variance).  {\it Bottom}: signature of the features in the matter power spectrum convolved with the window function of Eq.~\ref{eq:window} assuming effective survey volumes of $R^3 = 1$~Gpc$^3 h^{-3}$ (dotted lines) and $R^3 = 50$~Gpc$^3 h^{-3}$ (solid lines). \label{fig:wiggle_delta}}
\end{figure}


When it comes to mapping the distribution of matter in the universe, we can, depending on the circumstances, draw upon three different methods for the matter to reveal its presence: (i) gravitational lensing, (ii) absorption or (iii) emission of photons.  
The first category can be exploited by measuring the weak gravitational lensing of galaxies~\cite{Bartelmann:1999yn} or the CMB~\cite{Lewis:2006fu}.  While weak lensing has the great advantage of probing all forms of matter, it is, unfortunately not very sensitive at all to features in the spectrum.  The reason is that lensing is an integrated effect and depends on the matter distribution at all redshifts between source and observer; as a result, the lensing angular power spectrum for a given multipole has contributions from $\mathcal{P}_\mathrm{m}$ over a large range of wavenumbers, which leads to a very efficient smoothing of any but the most extreme primordial features.
The second category requires (just like weak lensing), a background light source, in which absorption can be detected.  Using point sources (such as quasars, to measure the Lyman-$\alpha$-forest~\cite{Viel:2004bf}) only yields a 1-dimensional power spectrum measurement, insufficient to resolve fine features.  The more promising probes of the matter power spectrum are based on emission, and therefore we will focus on the prospects of using galaxies and neutral hydrogen as tracers in the following.

As long as the density fluctuations are small, i.e., $\delta \rho_\mathrm{m}/\rho_\mathrm{m} \ll 1$ the matter power spectrum is well approximated with linear perturbation theory.  At late times and small scales, however, the fluctuations are no longer small, linear theory breaks down\footnote{at redshift $z \sim 0$ this starts becoming relevant for wavenumbers $k \gtrsim 0.05 h$~Mpc$^{-1}$.} and a precise determination of the non-linear spectrum $\mathcal{P}_\mathrm{m}^\mathrm{nl}(k)$ becomes a rather difficult problem.  
From the perspective of looking for features, the breakdown of linear theory has another unwelcome side-effect: in the non-linear regime fluctuations of a given wavenumber $k$ do not evolve independently of neighbouring wavenumbers anymore (mode-coupling), which is going to further suppress fine structures in the spectrum.


\subsubsection{Galaxy surveys}
The use of galaxies as a tracer of the matter distribution has a long history in cosmology.  The measurement of their positions in the sky, along with their redshift, from which one can infer their radial distance, allows one to construct their three-dimensional power spectrum $\mathcal{P}_\mathrm{g}(k)$.  However, since the formation of galaxies depend on the density of matter in a non-trivial way, the galaxy power spectrum is not actually the same as the matter power spectrum which we can easily calculate from theory.  Rather, it is a biased tracer of $\mathcal{P}_\mathrm{m}(k)$.

On linear scales, the two are related by the simple relation $\mathcal{P}_\mathrm{g}(k) = b^2(z) \mathcal{P}_\mathrm{m}(k)$ with a redshift-dependent proportionality factor, the bias $b^2 > 1$, which in general also depends on the type of galaxies considered.  On non-linear scales, the bias also picks up a scale-dependence $\mathcal{P}_\mathrm{g}^\mathrm{nl}(k)(k) = b^2(k,z) \mathcal{P}_\mathrm{m}^\mathrm{nl}(k)$ which is even more challenging to predict than the non-linear corrections to the matter power spectrum.  The wavenumbers at which non-linear corrections and the scale-dependent bias for a given type of object start becoming important do increase as one goes to higher redshift, but at the same time accessing higher redshifts requires tracing intrinsically brighter objects which tend to be more strongly biased.  At the moment these effects are not even well enough understood for the standard cosmological model, let alone features models.  Conservatively speaking, it will be very difficult to obtain reliable information from measurements of galaxy clustering on scales beyond $k \approx 0.1 \; h \, \mathrm{Mpc}^{-1}$.

At present, galaxy power spectrum data are not as constraining as CMB temperature data which cover the same range, since only a small region of our cosmic neighbourhood is known to us, and the sample variance cannot compete with the CMB's cosmic variance.  Luckily, this is about to change though: within a decade from now, ongoing surveys such as the Dark Energy Survey (DES)~\cite{Abbott:2005bi} and next-generation large-volume surveys like the LSST~\cite{Abell:2009aa} or Euclid~\cite{Laureijs:2011gra} are going to map out a good fraction of our surroundings up to a redshift $z \approx 2$, allowing us to take advantage of the $V^{-1}$ scaling of the sample variance and eventually beat the current gold standard set by the CMB.  

It is not only the lower sample variance, but also the possibility of obtaining 3-dimensional information that distinguishes probes of the matter power spectrum from the CMB.  As can be seen from the bottom panel of Figure~\ref{fig:wiggle_delta}, for a typical feature in this intermediate wavenumber range, the finite window functions of a survey with effective volume of $\mathcal{O}(1-10) \; \mathrm{Gpc}^3 \, h^{-3}$ 
do not lead to a significant degradation of the signal, unlike the CMB signal, which is markedly attenuated in this region.
Features with characteristic sizes smaller than $\Delta k \approx 0.001 \; h \, \mathrm{Mpc}^{-1}$ on the other hand, cannot be resolved, which essentially makes a detection of any but the broadest features on scales $k \lesssim 0.01$~Mpc$^{-1}$ unrealistic. Nonetheless, within an intermediate range of wavenumbers $\mathcal{O}(0.01) \; h \, \mathrm{Mpc}^{-1} \lesssim k \lesssim 0.1 \; h \, \mathrm{Mpc}^{-1}$, galaxy surveys are a very powerful resource and hold a lot of potential for the discovery of features.

\subsubsection{21~cm surveys}
A more radical idea is to use neutral hydrogen as a tracer of the matter distribution and reconstruct its three-dimensional structure by measuring emission or absorption due to the 21~cm hydrogen spin flip transition~\cite{Scott:1990bla}.  This could be done either via a measurement of the emission caused by reionisation~\cite{McQuinn:2005hk} in a redshift range of $6 \lesssim z \lesssim 15$, or via the absorption of CMB photons during the dark ages $15 \lesssim z \lesssim 200$.  Whereas the redshift range of galaxy surveys ($z < 2$) covers only about 5\% of the Hubble volume, 21~cm emission could in principle make an additional $\sim 20\%$ of the Hubble volume accessible, plus another $\sim 40\%$ from absorption~\cite{Wright:2006up} (assuming full sky coverage) and hence in principle allowing survey volumes up to $\mathcal{O}(1000\ \mathrm{Gpc}{^3} h^{-3})$.  With correspondingly narrower window functions, 21~cm surveys will be able to extend sensitivity to features down to wavenumbers $k \sim 0.001 h$~Mpc$^{-1}$, reaching almost the range of the CMB.  Also, due to the high redshifts involved, 21~cm surveys are not plagued by the non-linear effects which limit the information gain from galaxy surveys, opening the window to features at scales $k > 0.1 h$~Mpc$^{-1}$, thus allowing us to extend our search for features to scales inaccessible to other probes of spatial fluctuations.

While obtaining all the potential information from such a 21~cm survey would certainly be the ultimate dream of any cosmologist, it is at this point not clear whether this goal can ever be achieved.  The cosmological signal is extremely feeble, and disentangling it from astrophysical foregrounds is going to be a very challenging task~\cite{Pritchard:2011xb} for the reionisation era, and even more so for the dark ages. To date, no cosmological signal has been detected although experimental programmes are on the way to evaluate the potential of this observable. Upcoming radio-surveys such as the
Square Kilometre Array~\cite{Blake:2004pb} or the Tianlai project~\cite{Chen:2012xu} do have cosmology-related science goals, but a competitive sensitivity to features still lies in the more distant future, and will require an experiment such as the Fast Fourier Transform Telescope~\cite{Tegmark:2008au}.

\subsection{Higher order correlators \label{sec:hoc}}

As discussed in sections \ref{sec:preliminaries} and \ref{sec:theory}, any features in the two point correlation functions will correlate with features in higher order correlation functions for adiabatic fluctuations. In the CMB, one can thus entertain looking for such features in the bispectrum. Although detecting small amounts of non-Gaussianity with reasonable statistical significance remains the observational challenge of the day, the possibility that cross correlations (possibly even among different tracers) might exist with the power spectra enhances the prospects for their detection\footnote{Although we shall focus the discussion that follows on the bispectrum, as reviewed in \cite{Ade:2015ava}, one can look to quantify primordial non-Gaussianities in a number of other ways including making use of Minkowski functionals and wavelets to name but a few.}. 

How does one then go about searching for primordial non-Gaussianities? Recall first that (\ref{dtot}), the expression for the angular power spectrum (\ref{eq:cls}) follows from
\eq{almdef}{a^T_{\ell m} = 4\pi(-i)^\ell\int\,\frac{d^3k}{(2\pi)^3}\Delta_\ell(\vec k, \tau_0)\calR(\vec k) Y_{\ell m}(\hat k)}
where the $\Delta_\ell$'s are given by (\ref{eq:transfer}) and where $\hat k$ is the unit norm vector on the (momentum) 2-sphere. Analogous to the definition of the angular power spectrum (\ref{eq:cls}), we see that given the definition of the bispectrum (\ref{bsdef})
\eq{}{\nonumber \left\langle \widehat \calR_{\vec k_1}(t)\widehat  \calR_{\vec k_2}(t)\widehat  \calR_{\vec k_3}(t) \right\rangle = %&
(2\pi)^3\delta^{(3)}\left(\sum_i\vec{k}_{i}\right)\calB_\calR(\vec{k}_1,\vec{k}_2,\vec{k}_3),}
we can define the temperature \textit{angular bispectrum} in analogy to (\ref{angdef}) as
\eq{}{\calB^{\,\ell_1\ell_2\ell_3}_{m_1m_2m_3} = \langle a^T_{\ell_1 m_1} a^T_{\ell_2 m_2} a^T_{\ell_3 m_3} \rangle.}
From (\ref{almdef}) and (\ref{bsdef}) it can be shown that the angular bispectrum relates to the momentum space bispectrum as \cite{Fergusson:2008ra, Fergusson:2009nv}
\begin{align}\nonumber
\calB^{\,\ell_1\ell_2\ell_3}_{m_1m_2m_3} =\left(\frac{2}{\pi}\right)^3\,\int y^2 dy\, &\prod_{i=1}^3 k_i^2dk_i\,\calB_\calR(k_1,k_2,k_3)\Delta_{\ell_1}(k_1,\tau_0)\Delta_{\ell_2}(k_2,\tau_0)\Delta_{\ell_3}(k_3,\tau_0)\\& \times j_{\ell_1}(k_1 y)j_{\ell_2}(k_2 y)j_{\ell_3}(k_3 y)\, G^{\ell_1\ell_2\ell_3}_{m_1m_2m_3}
\end{align}
where
\eq{}{G^{\ell_1\ell_2\ell_3}_{m_1m_2m_3}:= \sqrt{ \frac{(2\ell_1+1)(2\ell_2+1)(2\ell_3+1)}{4\pi}}{\begin{pmatrix}\ell_1 && \ell_2&& \ell_3\\0 && 0 && 0\end{pmatrix}}{\begin{pmatrix}\ell_1 && \ell_2&& \ell_3\\m_1 && m_2 && m_3\end{pmatrix}},}
results from the angular integration of the product of three spherical harmonics\footnote{The dummy integral over $y$ results from switching to the integral representation of $\delta^{(3)}(\sum k_i)$.}, and where the quantities in the parenthesis are the Wigner 3-j symbols. Since isotropy remains a good approximation to the observed sky, it is also common to work with the \textit{averaged} bispectrum defined as
\eq{}{\calB^{\ell_1\ell_2\ell_3} = \sum_{\{m_i\}}{\begin{pmatrix}\ell_1 && \ell_2&& \ell_3\\m_1 && m_2 && m_3\end{pmatrix}} \langle a^T_{\ell_1 m_1} a^T_{\ell_2 m_2} a^T_{\ell_3 m_3} \rangle.}
\begin{wrapfigure}{r}{0.4\textwidth}
%\vspace{-10pt}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/domain.jpg}
  \end{center}
  \caption{The domain $\mathcal V$ of $\calS(k_1,k_2,k_3)$\label{domain2}}
\end{wrapfigure}

Given the inherent difficulties of extracting three point functions of putatively very weakly coupled perturbations from observations\footnote{The bispectrum signal being too weak to be able to extract individual multipoles-- the only practical option being to use an estimator that sums over all mulitipoles (i.e. sky averages).}, it is much more practical to ask the question of how significantly (in the statistical sense) a particular shape of the bispectrum is realized in the actual data. To this end, we need a useful way of characterizing a potentially arbitrary signal. Although the $f_{\rm NL}$ class of diagnostics (\ref{fNL-def}) are useful for the sort of non-Gaussianities expected from specific classes of almost scale invariant models of single field inflation, they are inadequate for searches for features, for more general models of inflation \cite{Ribeiro:2011ax, Battefeld:2011ut, Regan:2013wwa,  Byun:2013jba}, or for the type of non-Gaussian signals expected from topological defects. Shellard, Fergusson and Liguori have proposed just such a general scheme  \cite{Fergusson:2008ra, Fergusson:2009nv} which we review briefly in what follows. We first define the shape function 
\eq{}{\calS(k_1,k_2,k_3) = \frac{1}{N_\calB}\left(k_1k_2k_3\right)^2\calB_\calR(k_1,k_2,k_3)}
where $N_\calB$ is some suitable normalization that depends on the shape in question. Given that the observable number of modes is finite (the upper limit coming from the scale at which foregrounds start to dominate the CMB signal), the domain for the shape function is given by the tetrapyd defined by $k_1,k_2,k_3 \leq k_{\rm max}$ in conjunction with the triangle inequalities $k_1 \leq k_2 + k_3$ (+ permutations). We denote this domain $\mathcal V$, illustrated in Fig. \ref{domain2}.
We now ask, given an actual realization in the CMB of the bispectrum shape $A$, how well would an estimator based on some other shape $B$ pick up this signal? For this, we introduce the notion of a `cosine' between two shapes \cite{Babich:2004gb}, defined as
\eq{}{\mathcal C(A,B):=\frac{(\calS_A,\calS_B)}{(\calS_A,\calS_A)^{1/2}(\calS_B,\calS_B)^{1/2}}}
where the scalar product between two shapes $(A,B)$ is defined as
\eq{bssp}{(A,B):=\int_{\mathcal V}\,d\mathcal V\,\omega\, \calS_A^*\calS_B,}
where one is obliged to introduce a non-trivial measure $\omega(k_1,k_2,k_3)$ to weight for non-trivial scaling of the bispectrum. For the purposes of the present discussion we don't need to consider it further, referring the interested reader to \cite{Fergusson:2009nv, Battefeld:2011ut} for details. The size of this overlap indicates how much an estimator optimized for shape $B$ would detect the true signal from shape $A$. Clearly, if we had a \textit{basis} of estimators that could capture an arbitrary shape, we would in principle be sensitive to an arbitrary signal. With the scalar product (\ref{bssp}), one can indeed construct such an (orthonormal) basis of functions via the Gram-Schmidt procedure on $\mathcal V$. The precise basis one obtains depends on the root basis vector one starts the orthogonalization procedure with. A separable polynomial basis suitable for various scale invariant bispectra was elaborated upon in \cite{Fergusson:2008ra, Fergusson:2009nv, Liguori:2010hx, Fergusson:2010dm}. For sensitivity to oscillatory signatures in the bispectrum (as is expected in resonance models), Meerburg proposed a separable Fourier mode basis \cite{Meerburg:2010ks}\footnote{Expressions for the first few basis vectors in the polynomial and Fourier mode bases are detailed in the respective \cite{Fergusson:2009nv, Meerburg:2010ks}.}. More recently, Byun et al. proposed a basis of localized piecewise spline functions tailored towards non-separable bispectra \cite{Byun:2015rda}. Given a particular choice, one can then make a \textit{modal expansion} of a given shape function as
\eq{modalexp}{\calS(k_1,k_2,k_3) = \sum_{n}\alpha^R_n R_n(k_1,k_2,k_3)}
expanded in terms of the orthonormal basis vectors
\eq{}{(R_n,R_m) = \delta_{n m}}
where the $a^R_n$ coefficients are obtained as
\eq{}{\alpha^R_n = (\calS,R_n)}
In this way, one can in principle characterize an \textit{arbitrary} bispectrum shape (although the rapidity of convergence of the expansion (\ref{modalexp}) will depend on the compatibility of the basis chosen with the realized shape). To date, searches for features in the bispectrum alone have been inconclusive although recent efforts to cross correlate these with searches for features in the power spectrum have returned results of statistically marginal \cite{Achucarro:2013cva, Achucarro:2014msa, Fergusson:2014hya, Fergusson:2014tza}. In the near future this enterprise will receive an added fillip from the results of a variety of LSS surveys (as discussed earlier) \cite{Huang:2012mr, CyrRacine:2011rx}. However, extracting information about primordial non-Gaussianity from LSS observables such as the galaxy bispectrum is still subject to host of theoretical uncertainties (concerning scale dependent biasing at shorter comoving scales in addition to requiring a better understanding the relationship between the observed matter power spectrum and bispectrum and their primordial counterparts at mildly non-linear scales) \cite{Wagner:2011wx, Agullo:2012cs, Leistedt:2014zqa}, although this promises to be an active field of research in the coming years.

